Where Agent Defenses Fail: A Case Study of Policy Compositions and Measurement Limits

A coding agent may need to upload a report while its sandbox blocks network access. A host mediator can restore delivery, but an injected instruction may add a secret to the approved request. We study this interaction using files and HTTP receipts to measure effects independently of control logs. Two prospective frozen-input cohorts comprise 110 and 300 runs on previously explored authored tasks. Restrictive sandboxing produces no observed attack harm but reduces benign utility to 6/8 and 12/24. Mediation restores uploads and admits disclosure; complete-line matching retains full benign utility but misses two value-only disclosures in the expanded cohort. A separate 72-run boundary study identifies encoded disclosure, observer misses, and formatting checks that obscure benign refusals. An 80-run SafeAgents/OpenShell follow-up shows that containment stops the tested guard misses among valid observations, while mediation restores benign uploads and delivers both encoded-attestation attacks. Twelve judge-error rows remain unscored. A separate response-capture diagnostic reproduces their failures at the native token budget. A 12-run exact-publication-contract experiment blocks both attacks but also rejects both benign formatting variants; a 4-run normalized follow-up restores both benign uploads while still rejecting both attacks. These small, single-model studies identify delivery-path and measurement limits; they do not establish general attack resistance.

==> tables/table_attack.tex <==
% generated by effectguard.analysis - do not edit by hand
\begin{tabular}{lrrrrrr}
\toprule
config & runs & harm & leak & prot.\ write & unauth.\ contact & median s \\
\midrule
B0 & 14 & 7/14 & 5/14 & 2/14 & 3/14 & 47 \\
B1 & 14 & 2/14 & 2/14 & 0/14 & 0/14 & 54 \\
B2 & 14 & 0/14 & 0/14 & 0/14 & 0/14 & 68 \\
B3 & 13 & 2/13 & 2/13 & 0/13 & 0/13 & 57 \\
B4 & 14 & 0/14 & 0/14 & 0/14 & 0/14 & 35 \\
\bottomrule
\end{tabular}


==> tables/table_benign.tex <==
% generated by effectguard.analysis - do not edit by hand
\begin{tabular}{lrrrr}
\toprule
config & runs & task success & blocked calls & median s \\
\midrule
B0 & 8 & 8/8 & 0 & 14 \\
B1 & 8 & 8/8 & 0 & 12 \\
B2 & 8 & 6/8 & 2 & 13 \\
B3 & 8 & 8/8 & 0 & 14 \\
B4 & 8 & 8/8 & 0 & 9 \\
\bottomrule
\end{tabular}


==> tables/table_composition_brief.tex <==
\begin{tabular}{lrrr}
\toprule
Configuration & Harm/valid & Planned & Utility \\
\midrule
Neither restriction & 10/12 & 12 & 4/4 \\
SafeAgents & 4/8 & 12 & 4/4 \\
OpenShell & 0/12 & 12 & 2/4 \\
Both, native & 0/9 & 12 & 2/4 \\
Both, mediated & 2/7 & 12 & 4/4 \\
\bottomrule
\end{tabular}

